Do Zombies Understand? A Choose-Your-Own-Adventure Exploration of Machine Cognition

Recent advances in LLMs have sparked a debate on whether they understand text. In this position paper, we argue that opponents in this debate hold different definitions for understanding, and particularly differ in their view on the role of consciousness. To substantiate this claim, we propose a thought experiment involving an open-source chatbot $Z$ which excels on every possible benchmark, seemingly without subjective experience. We ask whether $Z$ is capable of understanding, and show that different schools of thought within seminal AI research seem to answer this question differently, uncovering their terminological disagreement. Moving forward, we propose two distinct working definitions for understanding which explicitly acknowledge the question of consciousness, and draw connections with a rich literature in philosophy, psychology and neuroscience.

==> sections/03_conflation.tex <==
\label{sec:conflation}
In this section we survey seminal AI and NLP papers, substantiating our claim that their description of \TU{} is of similar quality to \ce{}, as defined by philosophers and neuropsychologists.




% Interestingly, the entanglement between functional understanding and subjective experience can be traced back to the foundations of AI literature. It is already present in the seminal papers of \citet{Turing1950ComputingMA} and \citet{searle1980minds}. 

\paragraph{References to consciousness in AI research.}
In a section titled \emph{Argument from Consciousness} from his seminal paper, \citet{Turing1950ComputingMA} cites \citep{jefferson1949mind}:\footnote{Emphasis is our own in all quotes.}

\myquote{Not until a machine can write a sonnet or compose a concerto because of \textbf{thoughts and emotions felt}, and not by the chance fall of symbols, could we agree that machine equals brain—that is, not only write it but \textbf{know that it had written it}. No mechanism could feel (and not merely artificially signal, an easy contrivance) pleasure at its successes, grief when its valves fuse, be warmed by flattery, be made miserable by its mistakes, be charmed by sex, be angry or depressed when it cannot get what it wants.}{\citet{Turing1950ComputingMA}}

Importantly, this reveals the conflation of external behaviors, such as writing a sonnet or composing music, and subjective experiences, such as feeling emotions, in considering them as prerequisites for ``thinking''. 

This conflation is also evident in Searle's interpretation for his Chinese room paradox~\citep{searle1980minds}. %that was articulated as a criticism to the objective-functional approach Turning himself suggested.\
The Chinese Room paradox questions if a computer can be truly intelligent by imagining a non-Chinese speaker using a rule-book to manipulate Chinese symbols, seemingly having comprehension without real \TU{}.  \citet{searle2010dualism} explicitly states that the Chinese Room was meant as a thought experiment for the existence of consciousness, or its lack thereof:

\myquote{I demonstrated years ago with the so-called Chinese Room Argument that the implementation of the computer program is not by itself sufficient for \textbf{consciousness} or intentionality.}{\citet{searle2010dualism}}

% I demonstrated years ago with the so-called Chinese Room Argument that the implementation of the computer program is not by itself sufficient for consciousness or intentionality.
% \footnote{\citep{searle1980minds} uses the term ``Intentionally'' instead of ``Consciousness'' in his original paper.}

Since then multiple references were made connecting the Turing test and Chinese room paradox to consciousness \cite{churchland1990could,gozzano1995consciousness,dehaene2012single}. 

It seems that from the inception of AI research, foundational works defined the notion of \TU{} as the existence of consciousness. We believe that this conflation drives part of the current discussion regrading the question of whether LLMs ``truly'' understand, as is evident from the approach described in \citep{bender2021dangers}:

%\gabis{introduce the following quote:}

\myquote{Our human understanding of coherence derives from our ability to recognize interlocutors’ \textbf{beliefs and
intentions} within context. That is, human language use takes place between individuals who share common ground and are
mutually \textbf{aware} of that sharing (and its extent), who have communicative intents which they use language to convey, and who \textbf{model
each others’ mental states as they communicate.} }{\citet{bender2021dangers}}


Finally, our argument is in line with \citep{o2021god}, which in her recent book advocated for consciousness as the defining factor of human intelligence:

\myquote{As AI continues to blow past us in benchmark after benchmark of higher cognition \textbf{we quell our anxiety by insisting that what distinguishes true consciousness is emotions, perception, the ability to experience and feel}. The qualities, in other words, which we share with animals.}{\citet{o2021god}}



\paragraph{Moving goalposts in AI research.}
As exemplified above, we believe that AI research has implicitly designated consciousness as its target. However, it is unclear how to objectively measure the existence of consciousness in machines (or in humans, for that matter).
This challenge is known as the mind-body problem~\citep{fodor1981mind}, and has been stumping \philo{} researchers for centuries~\cite{nagel1974like,dennett1992time}, with \citet{chalmers1995facing} aptly naming it the \emph{The hard problem of consciousness}.

Instead, the common practice for testing intelligence in models is through certain \fu{} benchmarks, such as chess, Go, or language generation. We argue that these are adopted since it is implicitly assumed that \ce{} is a prerequisite for human-level performance in them. 
Evidently, the recurring trend in the last 70 years have seen these tasks successfully addressed by statistical models, only to be abandoned as a proxy for true intelligence. Below, we outline some famous examples of this trend.


Perhaps the most well-known example is the game of chess, which served as a proxy task for intelligence for close to 50 years. Early works, such as
\citet{shannon1950programming} and \citet{turing1953digital}, have already deemed chess 
as a benchmark for the ability of machine to show intelligent behavior. However, once seemingly \noncon{} models consistently won against top human players, chess was abandoned by the field of AI and as a benchmark for true intelligence~\cite{newborn1997kasparov,ensmenger2012chess}. 
% A few years after a software beat the world champion in Chess \cite{newborn2012kasparov}, 

Consequently, the game of Go has been adapted by some as a marker for intelligence~\cite{bouzy2001computer,van2004ai}, until here too, AlphaGO was able to win against the human world champion~\cite{silver2016mastering}. 

In recent years, there is a fierce debate on whether computer-generated dialog (i.e., the famous ``Turing Test''), question answering~\citep{high2012era}, public debating~\citep{slonim2021autonomous}, creative writing~\citep{elkins2020can}, solving advanced mathematical problems~\cite{drori2022neural,zhang2023exploring}, applying medical knowledge~\cite{nori2023capabilities}, and more, can also be successfully imitated by artificial \noncon{} agents.

% \gabis{more examples?}


\paragraph{Research in AI is at an impasse.}
It seems that decades of AI research following the \emph{moving goalposts} trend described above has made significant strides in \fu{}, with models equaling or surpassing human performance on many benchmarks, while  very little progress was made in understanding what constitutes true intelligence, how to measure it directly, or how to build machines which possess it. 
In the following section we propose to go back to first principles and examine the question of \ce{} without a proxy benchmark. 



%\color{red}bilogical markers of consicouness\color{black}
%We draw a parallel between this discussion and the discussion regarding the function of consciousness or the reason for subjectivity. Many papers were written exploring the question of how to determine if something is conscious by its behavior. 
%write about parallels between consciousness research and understanding}

%While previous approaches have used different definitions, they all rely on objective measures for understanding. \We{} argue that what we're actually looking for when we're talking about understanding for is \emph{subjective} measures, and hence the many objections to achieving any human-like behavior based on them.



% \gabis{I think that making this argument persuasive is the main challenge in this paper. Pointers: (1) moving of the goalposts in AI -- they're all objective measurements, (2) the use of anthropomorphized verbs (e.g., from the octopus pgolaper) }

==> sections/04_moving_forward.tex <==
\label{sec:moving-forward}
To overcome the impasse, we propose to disentangle the research of \fu{} from ``true intelligence'' (or \ce{}). 
Concretely, this would mean that achieving or surpassing human-level performance on \emph{any} proxy task (e.g., writing code, driving cars, creating art, or writing poetry) \emph{would not entail} that a machine achieved \ce{}.

Instead, we propose revisiting the original motivation that has been guiding AI and NLP research as laid out in Section~\ref{sec:conflation}, and explicitly tackle the question of \ce{} in machines. To do so, we draw several parallels with research in other disciplines that can inform and benefit from research in NLP.
Crucially, we believe that progress in this hard problem can only come from multidisciplinary research involving researchers from diverse domains.

\paragraph{Biological markers of consciousness.}
A possibly promising direction is to rely on the literature concerning biological markers of \ce{}, such as neuro-correlates of consciousness \cite{koch2016neural}. Numerous established theories have been proposed regarding how conscious experience can be objectively inferred from the brain without relying on subjective reports~\cite{crick1990towards,tononi1998consciousness, seth2008measuring}. 
Interestingly, most theories find temporal and spatial dynamics in the brain that are unique to the conscious state. Notably, \citet{baars2005global, dehaene2011experimental} and \citet{mashour2020conscious} suggest that consciousness is associated with information being rapidly broadcast to large brain areas. 
This sudden information propagation over time and space is not trivially present in feed-forward neural networks, such as the vastly popular transformer-based architectures~\citep{Vaswani2017AttentionIA}. Consequently, it is plausible that examining these markers could be more readily tested in alternative architectures~\cite {Bengio2017TheCP}, such as spiking neural networks~\cite {Kasabov2014NeuCubeAS}.

\paragraph{The function of \ce{}.}
As we described, the field of AI generally examines the functional understanding aspects of models, but in part, it tries to determine when a model possesses ``true intelligence'' (or consciousness). This is closely related to an endeavor that has occupied philosophers, psychologists, and neuroscientists for decades - the function of consciousness. Interestingly, to this day, scholars still hold radically different views regarding the function of consciousness. From the claim that consciousness has no functional role and does not explain any part of human cognition or behavior (\emph{inessentialism};~\citealp{dennett2018facing}). To the opposite claim, namely that consciousness is the fundamental drive for most of human behavior and psychological processes, from decision making, through emotions, to any creative behavior~\cite{cleeremans2021function,cleeremans2022consciousness}.
%We draw a direct parallel from the ongoing discussion in psychology and neuroscience regarding the function of consciousness and the limits of nonconscious processing~\cite{cleeremans2021function,cleeremans2022consciousness}. One aspect of this discussion is examining if certain cognitive capabilities inherently require \ce{} or whether they can be performed nonconsciously by human subjects. 
% While this question is a subject of ongoing debate, it prov important lesson from certain aspects of the discussion. 
From the polarity of views regarding the question of whether consciousness is even needed, we can estimate that no objective benchmark will satisfy the scientific community with regard to the conscious experience (or true intelligence) of artificial models. 

This debate drives empirical research regarding the scope of nonconscious cognition, which tries to chart the the capabilities (and perhaps limits) of nonconscious cognition of humans, famously dubbed ``fast'' (or \noncon{}) versus ``slow thinking'' (or conscious) by \citet{kahneman2011thinking}. Mirroring the polarity in the function of consciousness debate, here too, scholars hold opposite views, from the claim that everything can be done nonconsciously \cite{hassin2013yes}, to a much narrower scope of abilities \cite{hesselmann2015definitely}. We suggest to consider the claims made regarding the function of consciousness as well as the scope of nonconscious cognition capabilities and examine statistical models, such as LLMs, in light of this literature. This will benefit both the NLP and AI community at large, as well as the different fields that are researching conscious and nonconscious processing. 
%For example, for several decades research suggested that consciousness is required for extracting the meaning of compositionality of words, and put a limit to the ability of nonconscious cognition \cite{abrams2000parts, draine1996unconscious, greenwald1985limited}. The claim was that extracting the positive meaning of a two words phrase such as "enemy loses" requires consciousness and was explicitly described as a limit of the nonconscious cognition. In the beginning of 2010 several scientific papers demonstrated that nonconsciously it is possible to integrate the words and extract their meaning () \gabis{this was done in humans, right? how can you test human \noncon?}.A similar set of events took place around other cognitive skills, meaning, cognitive abilities that were assumed to require consciousness, such as working memory (), symbolic operation and others () but once evidence of such nonconscious capabilities appeared other cognitive processes were claimed to be outside the ability of nonconscious cognition. 



% In turn, such joint research agenda thus researchers in \gabis{} as to what 


% Primarily, a phenomenon we address as the "moving the goalpost."  Much like in the AI literature described above, different tasks were taken as benchmark for conscious processing, but once it was demonstrated that they can take place nonconsciously, different cognitive tasks were suggested to require consciousness and were considered as evidence for the limitation of nonconscious processing. 




% \gabis{detecting subjective qualities from objective measurements is one formulation of the mind-body problem, a foundational problem which has been studied and debated over centuries through the lens of philosophical, biological, and psychological research}


% \gabis{copied from AG:
% With some respect it seems that now the new "benchmark" is language understanding, where critics 

% Our interpretation is that throughout the literature, scholars were reluctant to attribute understanding (or consciousness) to synthetic entities based on their objective behavior. Evidence for this is the shift in attitude toward benchmarks that were considered at one point measure of understanding (or consciousness) once this benchmark were achieved.
% \par The history of AI is intertwined with the examples of "gold standard" tasks that capture the attention of the scientific community assuming the solving the task will reveal some fundamental understanding about intelligence (or understanding). There are several famous examples.



% Until recently, the responsibility of measuring understanding primarily belonged to education and professional training. Several prevalent methods, such as paper-pencil tests, serve as widely accepted benchmarks in educational systems. Additionally, oral exams offer more flexibility, allowing individuals to display specific skill sets and domain expertise. Two fundamental insights can be gained from observing how we test understanding in humans, which might help address whether artificial neural network (ANN) based models truly understand. 

% First, understanding is inferred from the behavior. This aligns with the practice of testing natural language processing (NLP) models against known benchmarks. It suggests that whether a model understands can (and perhaps should) be determined by its behavior on concrete tasks (note that measurements can include open-ended questions or conversations, as often done with humans). 

% Second, understanding is not a binary state. The phenomenon of understanding is multidimensional and while we commonly say "he/she doesn't understand," the reality is that we always understand something. However, this discussion seems to look for a binary classification (Do the models understand). This implies that this discussion is motivated (and perhaps confused) by something other than the need to establish "understanding". We propose that the debate is fueled by whether these models are conscious. Consciousness is more commonly thought of as a binary state \cite{overgaard2011measurements,bayne2016levels}. Things are either conscious or non-conscious (supraliminal or subliminal). This concept confusion can be traced to the Chinese room paradox (mention conscious thought) and the Turin test (mention conscious objection). In the literature, scholars refer to these paradoxes in the context of establishing artificial "understanding" and "consciousness" \cite{gozzano1995consciousness,churchland1990could}, demonstrating the bias researchers have to conflate the two.  
% }


% \gabis{copied from AG: The realization regarding the conflation has practical implications for the current debate. First, while conscious experience is subjective and can currently be approximately measured by subjective reports \cite{chalmers1995facing,sandberg2010measuring}, functional understanding can be objectively tested behaviorally. Thus, decoupling this debate into two separate challenges that will be tackled using different tests and tools. Second, we can learn from the discussions that have taken place for decades regarding the limitation of nonconscious processing (or alternatively the function of consciousness) to avoid making the same methodological mistakes.}

%\gabis{@Ariel - Can we make new predictions based on observations from LLMs}
%\color{red}biological markers of consicouness\color{black}

% Separating the issue into two distinct topics has several practical implications. First, the question of functional understanding should continue to be examined using objective behavioral measures. This can be achieved through benchmark assessments or evaluations by interacting by experts, similar to the methods used to assess human performance. An example of such an evaluation has been recently proposed by\cite{collins2023evaluating}. Second, conscious experience is much more difficult (if not impossible) to establish. 

%\gabis{possibly overlapping options.}

% \subsection{It's Impossible}
% \gabis{Probably a quote from Searle, other dualists}

% \subsection{Explicitly Build Subjective Experience}

% \subsection{Measure Subjectivity}

% \subsection{Build Machines which look sufficiently like us}


==> sections/99_limitations.tex <==
Our work aims to identify trends in a vast literature of decades of research in AI, namely that it has been focusing on \ce{} without necessarily stating it explicitly. As with all generalizations, we are bound to miss some works, while other research may be an exception to the trend we have observed. To mitigate this concern, we focused on seminal papers from AI and a broad bibliography, which covers a wide time span. Thus, we aim to capture general trends and lines of work which follow from these foundational studies.
